A Geometric Approach to On-road Motion Planning for Long and Multi-Body Heavy-Duty Vehicles

Driving heavy-duty vehicles, such as buses and tractor-trailer vehicles, is a difficult task in comparison to passenger cars. Most research on motion planning for autonomous vehicles has focused on passenger vehicles, and many unique challenges associated with heavy-duty vehicles remain open. However, recent works have started to tackle the particular difficulties related to on-road motion planning for buses and tractor-trailer vehicles using numerical optimization approaches. In this work, we propose a framework to design an optimization objective to be used in motion planners. Based on geometric derivations, the method finds the optimal trade-off between the conflicting objectives of centering different axles of the vehicle in the lane. For the buses, we consider the front and rear axles trade-off, whereas for articulated vehicles, we consider the tractor and trailer rear axles trade-off. Our results show that the proposed design strategy results in planned paths that considerably improve the behavior of heavy-duty vehicles by keeping the whole vehicle body in the center of the lane.

==> figures/tikz/draw_length_measure.tex <==
% This file defines the draw length measure command

\newcommand{\DrawLengthMeasure}[6]{
% #1 Start x
% #2 Start y
% #3 Final x
% #4 Final y
% #5 Measure angle (inferable from previous arguments, but easier if I just receive it )
% #6 Text to place

\coordinate (StartPoint) at ($(#1, #2)$);
\coordinate (FinalPoint) at ($(#3, #4)$);
%\coordinate (CornerFL) at ($ (#1, #2) + ({cos(#3)*#5-sin(#3)*#4}, {sin(#3)*#5+cos(#3)*#4})$);

\draw[fill=gray] (StartPoint) -- (FinalPoint);

\def\TickHalfLength{0.1}
\coordinate (StartPointA) at ($(#1, #2) + ({\TickHalfLength*cos(#5+90)},{\TickHalfLength*sin(#5+90)})$);
\coordinate (StartPointB) at ($(#1, #2) + ({\TickHalfLength*cos(#5-90)},{\TickHalfLength*sin(#5-90)})$);
\draw[fill=gray] (StartPointA) -- (StartPointB);

\coordinate (FinalPointA) at ($(#3, #4) + ({\TickHalfLength*cos(#5+90)},{\TickHalfLength*sin(#5+90)})$);
\coordinate (FinalPointB) at ($(#3, #4) + ({\TickHalfLength*cos(#5-90)},{\TickHalfLength*sin(#5-90)})$);
\draw[fill=gray] (FinalPointA) -- (FinalPointB);

\def\ExtraOffsetX{0.25*cos(#5+90)}
\def\ExtraOffsetY{0.25*sin(#5+90)}

\node[] at ($(StartPoint)!0.5!(FinalPoint) + ({\ExtraOffsetX}, {\ExtraOffsetY})$) {#6};  
%\draw[] (\ReferenceOriginX,\ReferenceOriginY)--(1.5,\ReferenceOriginY) node[right]{$x$};

}


==> figures/tikz/draw_radius_measure.tex <==
% This file defines the draw length measure command

\newcommand{\DrawRadiusMeasure}[6]{
% #1 Circle x
% #2 Circle y
% #3 Circle radius
% #4 Orientation of measure
% #5 Offset of text
% #6 Text to place

\coordinate (StartPoint) at ($(#1, #2)$);
%\coordinate (FinalPoint) at ($(#1 + #3*cos( #4 ), #2 + #3*sin( #4 ) )$);
\pgfmathsetmacro\FinalPointX{#1 + #3*cos( #4 )}
\pgfmathsetmacro\FinalPointY{#1 + #3*sin( #4 )}
\coordinate (FinalPoint) at ($(\FinalPointX , \FinalPointY )$);
%\coordinate (CornerFL) at ($ (#1, #2) + ({cos(#3)*#5-sin(#3)*#4}, {sin(#3)*#5+cos(#3)*#4})$);

\draw[fill=gray] (StartPoint) -- (FinalPoint);

\pgfmathsetmacro\OffsetText{#5}
\pgfmathsetmacro\FinalPointY{#1 + #3*sin( #4 )}

\pgfmathsetmacro\OffsetTextX{#5*cos(#4-90)}
\pgfmathsetmacro\OffsetTextY{#5*sin(#4-90)}

\node[anchor=north west] at ($(StartPoint)!0.5!(FinalPoint) + (\OffsetTextX, \OffsetTextY)$) {#6};  

}


==> figures/tikz/draw_trailer.tex <==
% This file defines the draw vehicle command

% Remember to add this line defining the \DrawWheel command in the parent file before calling this file.
% \input{\relativepathtikzfigure draw_wheel}

\newcommand{\DrawTrailer}[6]{
% #1 Vehicle x
% #2 Vehicle y
% #3 Vehicle theta
% #4 Vehicle half width
% #5 Vehicle front length
% #6 Vehicle rear length

\coordinate (CornerFR) at ($ (#1, #2) + ({cos(#3)*#5-sin(#3)*-#4}, {sin(#3)*#5+cos(#3)*-#4})$);
\coordinate (CornerFL) at ($ (#1, #2) + ({cos(#3)*#5-sin(#3)*#4}, {sin(#3)*#5+cos(#3)*#4})$);
\coordinate (CornerRL) at ($ (#1, #2) + ({cos(#3)*-#6-sin(#3)*#4}, {sin(#3)*-#6+cos(#3)*#4})$);
\coordinate (CornerRR) at ($ (#1, #2) + ({cos(#3)*-#6-sin(#3)*-#4}, {sin(#3)*-#6+cos(#3)*-#4})$);

\draw[fill=gray,very thick, fill opacity=0.4] (CornerFL) -- (CornerFR) -- (CornerRR) -- (CornerRL) -- cycle;


\def\AxleLength{#5-#6}

\coordinate (WheelRL) at ($ (#1, #2) + ({-sin(#3)*#4}, {cos(#3)*#4})$);
\coordinate (WheelRR) at ($ (#1, #2) + ({-sin(#3)*-#4}, {cos(#3)*-#4})$);

\def\WheelWidth{0.06}
\def\WheelHeight{0.125}

\DrawWheel{(WheelRL)}{#3}{\WheelWidth}{\WheelHeight}
\DrawWheel{(WheelRR)}{#3}{\WheelWidth}{\WheelHeight}


}


==> figures/tikz/draw_vehicle.tex <==
% This file defines the draw vehicle command

% Remember to add this line defining the \DrawWheel command in the parent file before calling this file.
% \input{\relativepathtikzfigure draw_wheel}

\newcommand{\DrawVehicle}[8]{
% #1 Vehicle x
% #2 Vehicle y
% #3 Vehicle theta
% #4 Vehicle half width
% #5 Vehicle axle length
% #6 Vehicle front length
% #7 Vehicle rear length
% #8 Steering wheel angle (degrees)



\coordinate (CornerFR) at ($ (#1, #2) + ({cos(#3)*(#5+#6)-sin(#3)*-#4}, {sin(#3)*(#5+#6)+cos(#3)*-#4})$);
\coordinate (CornerFL) at ($ (#1, #2) + ({cos(#3)*(#5+#6)-sin(#3)*#4}, {sin(#3)*(#5+#6)+cos(#3)*#4})$);
\coordinate (CornerRL) at ($ (#1, #2) + ({cos(#3)*-#7-sin(#3)*#4}, {sin(#3)*-#7+cos(#3)*#4})$);
\coordinate (CornerRR) at ($ (#1, #2) + ({cos(#3)*-#7-sin(#3)*-#4}, {sin(#3)*-#7+cos(#3)*-#4})$);

\draw[fill=gray,very thick, fill opacity=0.4] (CornerFL) -- (CornerFR) -- (CornerRR) -- (CornerRL) -- cycle;

\coordinate (WheelFR) at ($ (#1, #2) + ({cos(#3)*#5-sin(#3)*-#4}, {sin(#3)*#5+cos(#3)*-#4})$);
\coordinate (WheelFL) at ($ (#1, #2) + ({cos(#3)*#5-sin(#3)*#4}, {sin(#3)*#5+cos(#3)*#4})$);
\coordinate (WheelRL) at ($ (#1, #2) + ({-sin(#3)*#4}, {cos(#3)*#4})$);
\coordinate (WheelRR) at ($ (#1, #2) + ({-sin(#3)*-#4}, {cos(#3)*-#4})$);

\def\WheelWidth{0.06}
\def\WheelHeight{0.125}

\DrawWheel{(WheelFR)}{#3+#8}{\WheelWidth}{\WheelHeight}
\DrawWheel{(WheelFL)}{#3+#8}{\WheelWidth}{\WheelHeight}
\DrawWheel{(WheelRL)}{#3}{\WheelWidth}{\WheelHeight}
\DrawWheel{(WheelRR)}{#3}{\WheelWidth}{\WheelHeight}


}


==> figures/tikz/draw_wheel.tex <==
% This file defines the draw wheel command

\newcommand{\DrawWheel}[4]{
% #1 Wheel center coordinate
% #2 Wheel center y
% #3 Wheel theta
% #4 Wheel half width
% #5 Wheel half length

\coordinate (CornerFR) at ($ #1 + ({cos(#2)*#4-sin(#2)*-#3}, {sin(#2)*#4+cos(#2)*-#3})$);
\coordinate (CornerFL) at ($ #1 + ({cos(#2)*#4-sin(#2)*#3}, {sin(#2)*#4+cos(#2)*#3})$);
\coordinate (CornerRL) at ($ #1 + ({cos(#2)*-#4-sin(#2)*#3}, {sin(#2)*-#4+cos(#2)*#3})$);
\coordinate (CornerRR) at ($ #1 + ({cos(#2)*-#4-sin(#2)*-#3}, {sin(#2)*-#4+cos(#2)*-#3})$);

\draw[fill=black,very thick] (CornerFL) -- (CornerFR) -- (CornerRR) -- (CornerRL) -- cycle;

}

